D-DEMOS: A distributed, end-to-end verifiable, internet voting system

E-voting systems have emerged as a powerful technology for improving democracy by reducing election cost, increasing voter participation, and even allowing voters to directly verify the entire election procedure. Prior internet voting systems have single points of failure, which may result in the compromise of availability, voter secrecy, or integrity of the election results. In this paper, we present the design, implementation, security analysis, and evaluation of D-DEMOS, a complete e-voting system that is distributed, privacy-preserving and end-to-end verifiable. Our system includes a fully asynchronous vote collection subsystem that provides immediate assurance to the voter her vote was recorded as cast, without requiring cryptographic operations on behalf of the voter. We also include a distributed, replicated and fault-tolerant Bulletin Board component, that stores all necessary election-related information, and allows any party to read and verify the complete election process. Finally, we also incorporate trustees, i.e., individuals who control election result production while guaranteeing privacy and end-to-end-verifiability as long as their strong majority is honest. Our system is the first e-voting system whose voting operation is human verifiable, i.e., a voter can vote over the web, even when her web client stack is potentially unsafe, without sacrificing her privacy, and still be assured her vote was recorded as cast. Additionally, a voter can outsource election auditing to third parties, still without sacrificing privacy. Finally, as the number of auditors increases, the probability of election fraud going undetected is diminished exponentially. We provide a model and security analysis of the system. We implement a prototype of the complete system, we measure its performance experimentally, and we demonstrate its ability to handle large-scale elections.

==> demos.tex <==
\section{Case study: DEMOS e-voting system}
\subsection{DEMOS System Description}
In this section, we provide a high level description of DEMOS~\cite{DEMOS}, a state-of-the-art VCS that achieves end-to-end verifiability in the standard model for the first time.  
In DEMOS, each voter may select $1$ out of $m$ options and cast her vote using vote-codes listed in her ballot.
Each ballot has two functionally equivalent parts (with a complete list of the $m$ options in each part), instructing the voter to pick one of the two parts at random. 
The cryptographic payload tabulated on DEMOS's centralized BB consists of lists of the following primitives:
%\begin{itemize}
%\item 
\par\noindent\textbf{Additively homomorphic commitments:} where a value $M$ is posted in a committed form,
denoted by $\Com(M)$, such that (i) when the opening of $\Com(M)$ denoted by $\tilde{M}$ is posted, then no other value than $M$ can be extracted from $\tilde{M}$ (\emph{binding} property), (ii) $\Com(M)$ reveals no information about $M$ to any computationally bounded adversary (\emph{hiding} property) and (iii) for any two values $M_1, M_2$, it holds that $\Com(M_1) \cdot \Com(M_2) = \Com(M_1+M_2)$ (\emph{additive homomorphic} property).
%\item 
\par\noindent\textbf{Zero knowledge proofs:} these are proofs such that (i) if the honest verifier accepts a proof, then she is assured that the statement is true (\emph{soundness} property) and (ii) the proof reveals no other information than the truth of the statement (\emph{zero-knowledge property}). 
Specifically, DEMOS makes uses of \emph{three-move} zero-knowledge proofs, where the interaction is accomplished by a first move from the prover, a second move that is the verifier's challenge (the source of which is the random choice from the voters regarding the part of the ballot they chose), and a third move where the prover responds to the challenge which completes the proof.
%\end{itemize}
 

Formally, DEMOS consists of five protocols/algorithms: \textbf{Setup}, \textbf{Cast}, \textbf{Tally}, \textbf{Result}, and \textbf{Verify}. 
We will briefly present them here, omitting many cryptographic details, for simplicity.

In the \textbf{Setup} protocol, the EA generates the initialization data for each election entity.
More specifically, each randomly generated vote-code points to a cryptographic payload, consisting of additively homomorphic commitments of the \emph{option-encoding}, where the $i$-th option, $\mathsf{option}_i$, is encoded into $(n+1)^{i-1}$. 
These commitments are associated with necessary zero-knowledge proofs (prover's first move) that allow the EA to show that each commitment is valid  (i.e., it commits to an option encoding) later on, without revealing its actual content. 
The EA then assigns each ballot with two functionally equivalent parts. 
When the ballot preparation is finalized, the EA  distributes the ballots to the voters via BDS.\\
%
\indent In the \textbf{Cast} protocol, the voter randomly chooses one of the two parts of the ballot to vote by submitting the vote-code corresponding to her intended option. 
The unused part will be kept for auditing after the election ends. \\
 %
\indent In the \textbf{Tally} protocol, the EA fetches the entire election transcript from the BB and posts additional data on the BB. 
In this step, the tally result is produced using the homomorphic property by ``adding'' all the option-encoding commitments associated with the vote-codes cast by the voters and are marked as ``$\mathsf{voted}$''. Note that, the result is in committed form and requires the corresponding opening to be decoded.
Furthermore, the commitments that correspond to the unused parts of voter ballots are also revealed for auditing. 
Finally, the EA derives the challenge (second move) of the zero-knowledge proofs based on the voters' choices of used ballot parts and completes the zero-knowledge proofs that correspond to the option-encoding commitments marked as ``$\mathsf{voted}$'', by posting all the respective third moves of the prover.\\
%
\indent The \textbf{Result} algorithm takes as input the entire BB information, and can be executed by anyone. 
For instance, if $n=9$, the \emph{option-encodings} of options $1,2,3$ are $1,10,100$, respectively. 
Suppose we got $3$ votes for $\mathsf{option}_1$, $5$ votes for $\mathsf{option}_3$, the sum of the \emph{option-encodings} is $3*1+5*100=503$. 
By the opening of the homomorphic tally, the \textbf{Result} algorithm extracts $503$ and decodes it as $(3,0,5)$, which represents the corresponding votes for each election option.\\
%
\indent The \textbf{Verify} algorithm can be executed by voters and any third-party auditors. 
A third-party auditor is able to verify the validity of all the commitments by checking the completed zero-knowledge proofs.
Besides, each voter is allowed to perform ``print check'' by comparing her private ballot with the information on the BB.
As the number of auditing voters increases, the probability of election fraud going undetected diminishes exponentially.
For example, even if only $10$ voters audit, with each one having $1 \over 2$ probability to detect ballot fraud, the probability of ballot fraud going undetected is only ${1 \over 2}^{10} = 0.00097$.\\
%
\indent Notice that, in its current form, DEMOS is a centralized system. 
It depends on a consistent Bulletin Board for its functionality, and the EA is responsible for performing the \textbf{Setup}, collecting the cast votes and posting them to the BB, and playing the role of a single trustee entity which engages the \textbf{Tally} and \textbf{Result} protocols, to produce and publish the election result. 

\subsection{Distributing DEMOS}\label{subsec:dDemos}
In this section, we present a distributed version of DEMOS where we (i) integrate our DBB system with DEMOS and (ii) distribute the trustee functionality in the tally phase. As previously mentioned, our goals are two-fold. 
First, by using our VC nodes for vote collection, we increase the fault-tolerance of the voting phase, removing any single point of failure during election hours.
Additionally, by following the advice of the original publication, we remove the Tally and Result functionality from the EA, and assign it to  $N_{tr}$ ``trustee'' nodes, thus removing single points of failure even after election hours. 
To achieve this, we introduce \emph{verifiable secret sharing}, across trustee nodes, to share the opening of each option encoding commitment.
We require at least $k_{tr}$-out-of-$N_{tr}$ shares for the secret to be reconstructed.
With these additions, the EA is left only with the setup task, and thus can be ``destroyed'' immediately after it sets up the election, to reduce exposure to privacy attacks.


\subsubsection{Integrating our DBB with DEMOS}\label{subsubsec:dDemos-DBB}

%Henceforth, the whole voting system becomes completely distributed.

% Additionally, we split the EA into multiple entities, which we leave centralized for this case study.
% EA is now employed only during setup, as explained below. 
% We create a single \emph{Trustee} node, that takes over the \emph{Tally} and \emph{Result} functionality from EA.
% In the future, we plan to apply threshold cryptography techniques to split the single \emph{TrusteE} into multiple entities, cvommunicating only by reading and writing to our DBB, rendering the whole voting system completely distributed, beyond setup.


We modify the \textbf{Setup} protocol of DEMOS to a pre-processing component that is compatible with our distributed BB system. 
We let the existing \textbf{Setup} introduce election options, and produce their corresponding option-encodings, homomorphic option-encoding commitments and openings, for both parts of each ballot.
Then, DBB's TS attaches a vote-code and receipt to each line of every ballot and hands it back to DEMOS's BDS. 
%In its simplest form, a BDS for DEMOS can be a printer that prints paper ballots, which are physically distributed (out-of-band) to voters.\\
%To preserve the end-to-end verifiability of DEMOS, for $n$ voters, the pre-processing component $n$ $2m$-sized lists accompanied with unique $\mathsf{serial\textrm{-}no}_\ell$. 
% Each list consists of two sets of additively homomorphic commitments of option encodings (as well as the first move of the zero-knowledge proofs), i.e.,
% $
% \langle (\mathsf{option}_1,\mathsf{encoding}_i),\ldots, (\mathsf{option}_m,\mathsf{encoding}_m),\allowbreak (\mathsf{option}_1,\mathsf{encoding}_i),\ldots, (\mathsf{option}_m,\mathsf{encoding}_m) \rangle
% $. 
\indent The voters are instructed to use either the first half or the second half of the ballot to vote (following Alg.~\ref{alg:vote}) and keep the other half for auditing. 
Our DBB remains oblivious to the fact each ballot contains two functionally equivalent sections; to the DBB, it looks like the list of options for each ballot has size $L=2m$.

\subsubsection{Distributing the trustees in DEMOS}\label{subsubsec:dDemos-trustees}
At \textbf{Setup}, we enhance the EA to use a  $k_{tr}$-out-of-$N_{tr}$ verifiable secret sharing scheme, to share its internal state information (that contains the openings of every commitment and necessary information for completing all the zero-knowledge proofs on demand) to the $N_{tr}$ trustees. To implement \textbf{Tally}, trustees follow these steps:
\begin{enumerate}
 \item \label{trustee:etally} Each trustee will fetch the election transcript from the TAs, and determine the genuine tally set $E_\mathsf{tally}$, that consists of the commitments which have been marked as ``$\mathsf{voted}$'' (there is no need to write this back to TAs).
%, is determined as the majority of the election data posted on all the TA nodes.\\
 \item \label{trustee:esum} Each trustee computes and publishes $E_\mathsf{sum}$, which is the homomorphic tally in committed form.
 \item \label{trustee:share} Each trustee computes its share of the opening of the homomorphic tally by adding all its private shares of openings of the option-encoding commitments in  $E_\mathsf{tally}$.
 This is achievable because DEMOS has the nice attribute, that the opening of the sum can be calculated as the sum of each corresponding individual opening (that is, the homomorphic property extends to openings as well). 
 \item \label{trustee:zkp} Finally, the trustee will derive the challenge of the zero-knowledge proofs (following the same protocol as the centralized version), and generate the shares of the third move of the zero-knowledge proofs for the encodings in  $E_\mathsf{tally}$. 
\end{enumerate}

At each step, each trustee will update each TA node with the produced data.
%along with its shares of all option-encoding commitment openings to every TA node.

%\textcolor{blue}{\textbf{Note to Nikos:} the way we have it every write besides the zero knowledge proofs requires $k_{tr}$-out-of-$N_{tr}$ trustees. What should we do about the proofs? the TA is sure of the write when it receives more than $f_{tr}$ copies of a message, where $f_{tr}$ is the trustee fault tolerance.}
Procedure $VW$ is implemented as follows: writes are allowed only by trustees (verified by the keys, generated and supplied by DEMOS's EA). 
For steps~\ref{trustee:esum} and \ref{trustee:zkp}, where each trustee is expected to write the same data to each TA, $VW$ simply waits until $N_{tr} - k_{tr} + 1$ identical posts have been submitted, then allows publishing the posted data.
For step~\ref{trustee:share}, where each trustee submits different information, $VW$ waits for $k_{tr}$ valid posts from trustees, then runs a DEMOS specific calculation which allows the tally to be opened, and forwards the final result to the TA node for publishing.

%A write is accepted only when performed by $k$ out of $n$ trustees.
%\textcolor{green}{Please elaborate on what they post that is different from each other, so I can say $VW$ allows it when $k$ valid out of $n$ are posted (while until then, they are kept as private state inside $VW$)}

%After the election ends, the post-processing component of DEMOS will fetch the election transcript from each TA. 
%Use the most common view of them as the legitimate election transcript. 
%It first derive the challenge of the zero-knowledge proofs based on how the voters' choices, and then complete the second move of the zero-knowledge proofs. 
%The post-processing component then homomorphically add these commitments that has been marked as ``$\mathsf{voted}$'' and open the sum to produce the election tally. 
%Meanwhile, it also reveals the opening for those commitments that belong to the unused half of the voters' ballots.
%All these information will be posted back to each TA as the final election data.

% If any TA gives inconsistent election transcript (compared with the others), the post-processing component also marks it as ``$\mathsf{defected}$''. The defected TA list is also posted to all the TA at the end.
% Subsequently, all the voters as well as any third-party auditors can fetch election transcript from an honest TA to verify the integrity of the entire election.

\subsection{Properties of Distributed DEMOS}\label{subsubsec:dDemos-properties}
Our resulting Distributed DEMOS system preserves both the end-to-end verifiability and privacy properties of the centralized DEMOS.
\par\noindent\textbf{End-to-end verifiability. } Centralized DEMOS achieves end-to-end verifiability against an adversary that controls the entire election procedure (\cite[Theorem 4]{DEMOS}). Therefore, Distributed DEMOS preserves the same level of end-to-end verifiability against adversaries that may corrupt the EA, the TS, the BDS, all VC nodes, and all the trustees. 
In addition, the consistency of the view of the BB, which is the only requirement for end-to-end verifiability, is achieved by the fault tolerance threshold of the TA nodes.
%
\par\noindent\textbf{Voter privacy. } Centralized DEMOS achieves voter privacy against adversaries that observe the entire network traffic and obtain the voters' audit information (\cite[Theorem 5]{DEMOS}).  In this model, the EA, the VC and the trustees' subsystems  are merged in to a single honest authority. Adapting the proof to the system model described in Section~\ref{sec:model} is accomplished by (i) destroying the EA and DBB's TS (ii) the fault tolerance threshold of the VC and the trustees' subsystems and (iii) the fault tolerance threshold of the TA subsystem.

By integrating DEMOS with our DBB, the resulting system possesses the following extra properties:
\begin{itemize}
 \item It provides fault-tolerant long-term storage of election data, using our TA nodes.
 \item It provides fault-tolerant vote collection, during election hours, using our VC nodes.
 \item It provides immediate feedback to the voter, assuring her that her vote was recorded-as-cast, using our receipt mechanism. 
 In the original DEMOS system, the voter has to consult the BB after election hours, to verify her vote was recorded, a far more complex interaction for unsophisticated users.
\end{itemize}

Furthermore, by applying threshold cryptography and introducing \emph{trustees}, we eliminate all single points of failure, beyond the setup performed by the EA. Note that, due to the inherent end-to-end verifiability of DEMOS, a malicious setup by the EA can be detected using the \emph{Verify} algorithm. Thus, even the only remaining centralized component cannot lead to an undetected erroneous election result.
To our knowledge, Distributed DEMOS is the \textbf{first end-to-end verifiable web-based voting system without any single point of failure besides setup}.



==> proofmodel.tex <==
\section{Liveness and safety of our e-voting system}\label{subsec:secure}

\subsection{The adversarial model.}\label{app:proofmodel}
\ignore{
Let $N_\mathsf{v},N_\mathsf{b}$ and $N_\mathsf{t}$ be the number of VC nodes, ABB nodes and trustees respectively. The voters are denoted by $V_\ell$, $\ell=1,\ldots,n$. We assume that there exists a \emph{global clock} variable $\Cl\in\mathbb{N}$, and every node $X$ is equipped with an \emph{internal clock} variable $\Cl[X]\in\mathbb{N}$. We define the two following events to describe synchronization loss among the clocks caused by the adversary $\A$:
\begin{enumerate}[(i).]
 \item The event $\mathsf{Inc}(i):$ $i\leftarrow i+1$, that causes some clock $i$ to advance by one time unit.
 \item The event $\mathsf{Init}(X):$ $\mathsf{Clock}[X]\leftarrow\mathsf{Clock}$, that initializes a node $X$ by synchronizing its internal clock with the global clock. 
\end{enumerate}
The adversarial setting for $\A$ upon the distributed system $\mathbf{Sys}$ is defined in Figure~\ref{fig:threat}.
\begin{boxfig}{\label{fig:threat} The adversarial setting for the adversary $\A$ upon the distributed system $\mathbf{Sys}$.}{}
  {\it \underline{The adversarial setting.}}
\begin{enumerate}
 \item EA initializes every component node (VC node, ABB node or trustee) $X$ of $\mathbf{Sys}$ by running $\mathsf{Init}(X)$ for clock synchronization. Then, EA sets up the election and provides all the nodes (i.e. component nodes and voters) with their individual election information.
 \item $\A$ corrupts a fixed subset of VC nodes, a fixed subset of ABB nodes and a fixed subset of trustees. In addition, it defines a dynamically updated subset of voters $\mathbf{V}_\mathsf{corr}$, initially set as empty. 
 %Then, it provides $\mathsf{Sys}$ with $\mathbf{VC}_\mathsf{corr}$ and $\mathbf{V}_\mathsf{corr}$, which in turn will play the role of every non-corrupted node.
\item When an honest node $X$ wants to transmit a message $M$ to an honest node $Y$, then it just sends $(X,M,Y)$ to $\A$.
 \item $\A$ may arbitrarily invoke the events $\mathsf{Inc}(\mathsf{Clock})$ or $\mathsf{Inc}(\mathsf{Clock}[X])$, for any node $X$. Moreover, $\A$ may write on the incoming network tape of any honest component node of $\mathbf{Sys}$.
% \textcolor{teal}{\textbf{Thomas}: I did not include $\mathsf{Init}()$, as clocks cannot go back, right?}
 \item For every voter $V_\ell$, $\A$ can choose whether it is going to include $V_\ell$ in $\mathbf{V}_\mathsf{corr}$. 
 \begin{enumerate}[(i).]
  \item If $V_\ell\in\mathbf{V}_\mathsf{corr}$, then $\A$ fully controls $V_\ell$.
  \item If $V_\ell\notin\mathbf{V}_\mathsf{corr}$, then $\A$ may initialize $V_\ell$ by running $\mathsf{Init}(V_\ell)$ only once. If this happens, then the only control of $\A$ over $V_\ell$ is $\mathsf{Inc}(\mathsf{Clock}[V_\ell])$ invocations. Upon initialization, $V_\ell$ starts running the voting algorithm~\ref{alg:vote}.
 \end{enumerate} 
\end{enumerate}
\end{boxfig}
}
%-----------------------------------------------the game------------------------------------------------------------------------------------------
In order for our system to achieve liveness and safety, we have to restrict the adversarial setting in Figure~\ref{fig:threat} by requiring the following assumptions:
\begin{enumerate}
 \item The fault tolerance thresholds described in Section~\ref{subsec:threat}. Namely, $\A$ can corrupt up to: (1.a) $f_\mathsf{v}$ out-of $N_\mathsf{v}$ VC nodes, (1.b) $f_\mathsf{b}$ out-of $N_\mathsf{b}$ ABB nodes and (1.c) $f_\mathsf{t}$ out-of $N_\mathsf{t}$ trustees, where $N_\mathsf{v}\geq3f_\mathsf{v}+1$ and $N_\mathsf{b}\geq2f_\mathsf{b}+1$.
 \item There exists an upper bound $\Delta$ of the drift of all honest nodes' internal clocks with respect to the global clock. Formally, we have that: $|\mathsf{Clock}[X]-\mathsf{Clock}|\leq\Delta$  for every node $X$, where $|\cdot|$ denotes the absolute value.
 \item There exists an upper bound $\delta$ on the time that $\A$ can delay the delivery of the messages between honest nodes. Formally, when the honest node $X$ sends $(X,M,Y)$ to $\A$, if the value of the global clock is $t$, then $\A$ must write $M$ on the incoming network tape of $Y$ by the time that  
 $\mathsf{Clock}=t+\delta$.
  \item There exists a value $\mathsf{End}$ such that for each honest node $X$, if $\mathsf{Clock}[X]\geq\mathsf{End}$, then $X$ assumes that the voting phase has ended.
 \item There exists a positive value $D$ (that depends on the computational and network overhead of the system) such that 
for each honest VC node $X$, if $\mathsf{Clock}[X]\geq\mathsf{End}+D$, then $X$ starts computing its view of the set of votes to be tallied.
\end{enumerate}

\noindent The assumptions 1.a, 2, 3, 4 are sufficient for liveness. For safety, assumption 5 is additionally required to guarantee that the honest VC node $X$ proceeds to the Result Consensus phase of the IC protocol (see Section~\ref{section:ic}),%, where $X$ started participating in the Value Dissemination phase when $\mathsf{Clock}[X]=\mathsf{End}$. 





==> properties.tex <==
\subsection{Properties of our e-voting system}\label{subsec:properties}
In this section, we discuss how our e-voting system achieves the properties mentioned in Section~\ref{section:voteback}. Here we focus on fault-tolerance since this is our main objective. The other necessary properties, verifiability and privacy, have been shown in 
\cite{kiayias-eurocrypt-2015}. In more details:
%\subsubsection{End-to-end verifiability}\label{subsubsec:E2E}


\noindent\textbf{Fault tolerance. }%\label{subsubsec:tolerance}
The only component of our e-voting system that is not distributed as a subsystem is the EA since it is just an algorithm whose local state is erased immediately after the setup phase is completed. All the other components, i.e. the VC, ABB and trustees' subsystem, are distributed and resilient up to a number of faulty nodes, determined in Section~\ref{subsubsec:threat}. This resilience is crucial in order  for our system to achieve end-to-end verifiability, voter privacy and receipt freeness, as well as liveness and safety that we prove in Appendix~\ref{subsec:secure}.

\noindent\textbf{End-to-end verifiability. }The end-to-end verifiability that our e-voting system achieves is formalized in  \cite{kiayias-eurocrypt-2015} (Section 2.3) and proven in \cite{kiayias-eurocrypt-2015} (Theorem 4). Informally, our system is end-to-end verifiable against adversaries that may corrupt the EA, all VC nodes, and all the trustees. %and up to a number of voters. 
In addition, the consistency of the view of the ABB, which is the only requirement for end-to-end verifiability, is achieved by the fault tolerance threshold of the ABB subsystem. %(see Section~\ref{subsubsec:tolerance}).\\ %Namely, if up to $f_\mathsf{b}$ of the ABB nodes are malicious, where $N_\mathsf{b}\geq2f_\mathsf{b}+1$, then any party that reads from the ABB nodes, decides on the consistent view of the ABB simply by taking the honest majority.

\noindent\textbf{Voter privacy/Receipt-freeness. }%\label{subsubsec:privacy}
The voter privacy/receipt-freeness that our e-voting system achieves is formalized in  \cite{kiayias-eurocrypt-2015} (Section 2.3) and proven in \cite{kiayias-eurocrypt-2015} (Theorem 5). In this model, the EA, the VC and the trustees' subsystems  are merged in to a single honest authority. Adapting the proof to the system model described in Section~\ref{sec:model} is accomplished by (i) destroying the EA (ii) the fault tolerance threshold of the VC and the trustees' subsystems and (iii) the fault tolerance threshold of the ABB subsystem.



==> system-bc.tex <==
\subsection{Completely asynchronous version}
\label{sect:asyncConsensus}

The algorithms we presented so far for voting and vote set consensus are very efficient, a fact we establish in section~\ref{sect:evaluation}. 
Our voting protocol takes approximately a single round-trip of communication between the vote collectors, while the IC-based consensus causes the transfer of each node's vote set to every other node, and requires one binary consensus for each node's set.
However this comes at the cost of a timing assumption, rendering the system vulnerable to timing attacks at the specific time frame between election end (otherwise, the start of IC), and the \emph{barrier} establishing the end of the value dissemination phase of IC.

We have already improved our algorithms to remove this timing assumption, and we briefly present our solution here. 
We first introduce one more multicast round, \textbf{before} the responder VC node starts the round of multicasts, by sending the VOTE\_P message.
The purpose of this extra round is to guarantee the uniqueness of the used vote code per ballot; that is, that either only one vote code is stored by the majority of nodes before the voter's receipt is generated, or no vote code is stored at all. 
In this round, inspired by the Echo Multicast primitive introduced by Reiter in~\cite{reiter.secure}, the responder node sends an ENDORSEMENT\_REQUEST($serial\textrm{-}no,vote\textrm{-}code$) message to all VC nodes. 
Each receiving node $VC_i$ signs this message only if it knows of no other vote code for this ballot, and replies with an ENDORSEMENT\_RESPONSE($serial\textrm{-}no,vote\textrm{-}code,signature_i$).
The responder node gathers $N_v-f_v$ such endorsement responses into $UCERT$, the vote code's  uniqueness certificate. 

We then modify the VOTE\_P messages to include the $UCERT$ of the corresponding vote code. 
We also modify our algorithms to always verify the validity of $UCERT$ before any further processing of the VOTE\_P message. With these enhancements during the voting protocol, we can guarantee the following:
\begin{enumerate}[a)]
\item No matter how many responders and vote codes are active at the same time, if a $UCERT$ is formed for vote code $vc_a$, no other uniqueness certificate for any vote code different than $vc_a$ can be formed.
\item By verifying the $UCERT$ before disclosing a VC node's receipt share, we guarantee the voter's receipt cannot be reconstructed unless a valid $UCERT$ is present. 
\end{enumerate}

Now, at election end time, we don't use Interactive Consistency any more. Instead each VC node performs the following steps, for each ballot:
\begin{enumerate}
\item 
\label{bc-step-announce} 
Send ANNOUNCE($serial\textrm{-}no, vote\textrm{-}code, UCERT$) to all nodes. 
The vote-code will be \emph{null} if the node knows of no vote code for this ballot.

\item 
\label{bc-step-wait} 
Wait for $N_v-f_v$ such messages for this ballot. 
If any of these messages contains a valid vote code $vc_a$, accompanied by a valid $UCERT$, change the local state immediately, by setting $vc_a$ as the vote code used for this ballot.

\item 
\label{bc-step-bc} 
Participate in a Binary Consensus protocol, with the subject "Is there a valid vote code for this ballot?". 
Enter with an opinion of $1$, if a valid vote code is locally known, or a $0$ otherwise.

\item 
\label{bc-step-result-0} 
If the result of Binary Consensus is $0$, consider the ballot not voted. 

\item 
\label{bc-step-result-1} 
Else, if the result of Binary Consensus is $1$, consider the ballot voted. 
There are two sub-cases here: 
\begin{enumerate}[a)]
\item 
\label{bc-step-result-1-known} 
If vote code $vc_a$, accompanied by a valid $UCERT$ is locally known, consider the ballot voted for $vc_a$. 

\item 
\label{bc-step-result-1-unknown} 
If, however, $vc_a$ is not known, send a RECOVER-REQUEST($serial\textrm{-}no$) message to all VC nodes, wait for the first valid RECOVER-RESPONSE($serial\textrm{-}no, vc_a, UCERT$) response, and update the local state accordingly.
\end{enumerate}
\end{enumerate}

Steps~\ref{bc-step-announce}-\ref{bc-step-wait} ensure used vote codes are dispersed across nodes. 
Recall our receipt generation requires $N_v-f_v$ shares to be revealed by distinct VC nodes, of which at least $N_v-2f_v$ are honest. 
Now notice that any two $N_v-f_v$ subsets of $N_v$ have at least one honest node in common. Because of this, if a receipt was generated, at least one  honest node's announcement will be processed by every honest node. 
Consequently, if a receipt was indeed generated, all honest VC nodes will obtain the corresponding vote code in these two steps, and thus enter step~\ref{bc-step-bc} with an opinion of $1$.
In this case, binary consensus is guaranteed to deliver $1$ as the resulting value (because all honest nodes share the same opinion), thus safeguarding our contract against the voters.
%In any case, steps~\ref{bc-step-bc}-\ref{bc-step-result-1} ensure the system is coherent across all nodes.
In any case, step~\ref{bc-step-bc} guarantees all VC nodes arrive to the same conclusion, on weather this ballot is voted or not.

In the algorithm outlined above, the result from binary consensus is translated from $1$/$0$ to a unique valid vote code, or a status of ``not-voted'', in steps \ref{bc-step-result-0}-\ref{bc-step-result-1}. 
The~\ref{bc-step-result-1-unknown} case of this translation, in particular, requires additional justification. 
Assume, for example, that a voter submitted a valid vote code $vc_a$, but a receipt was not generated before election end time. 
In this case, an honest vote collector node $VC_A$ may not be aware of $vc_a$ at step~\ref{bc-step-bc}, as steps~\ref{bc-step-announce}-\ref{bc-step-wait} do not make any guarantees in this case. 
Thus, it may rightfully enter consensus with a value of $0$.  
However, when opinions are mixed, the consensus algorithm may produce any result.
In case the result is $1$, $VC_A$ will not possess the correct vote code $vc_a$, and thus will not be able to translate the result properly. 
This is what our recovery sub-protocol is designed for. 
$VC_A$ will issue a RECOVER-REQUEST multicast, and we claim that another honest node, $VC_B$ exists that possesses $vc_a$ and will reply with it. 
The reason for the existence of an honest $VC_B$ is straightforward and stems from the properties of the binary consensus problem's definition.
If all honest nodes enter binary consensus with the same opinion $a$, the result of any consensus algorithm is guaranteed to be $a$. 
Since we have an honest node $VC_A$, that entered consensus with a value of $0$, but a result of $1$ was produced, there has to exist another honest node $VC_B$ that entered consensus with an opinion of $1$. Since $VC_B$ is honest, is has to possess $vc_a$, along with the corresponding $UCERT$ (as no other vote code $vc_b$ can be active at the same time for this ballot). Again, because $VC_B$ is honest, it will follow the protocol and reply with a well formed RECOVER-REPLY. Additionally, the existence of $UCERT$ guarantees that any malicious replies can be safely identified and discarded by $VC_A$.

The modified voting and vote set consensus protocols presented in this section achieve the same end-result as the ones of section~\ref{subsec:Vcnodes}, without any timing assumptions. 
However, there is a significant performance penalty in this new approach, as one binary consensus instance is required \emph{for each ballot}.
Even at the minimum expected cost of $O(N_v^2)$ for a consensus algorithm, multiplying it with the number of ballots yields a large message complexity of $O(N N_v^2)$ ($N$ is the number of ballots).
This is why we are still investigating optimizations to these asynchronous algorithms, and we do not present a performance evaluation for them in this paper.


==> system.tex <==
\section{System description}
\subsection{Problem definition and goals}
We consider an \emph{election} with a single \emph{question} and $m$ \emph{options}, for a voter population of size $n$, where voting takes place between a certain \emph{begin} and \emph{end} time (the \emph{voting hours}), and each voter may select a single \emph{option}.

Our major goals in designing our voting system are three. 
First, it has to be end-to-end verifiable, so that anyone can verify the complete election process. 
Additionally, voters should be able to outsource auditing to third parties, without revealing their voting choice.
Second, it has to be fault-tolerant, so that an attack on system availability and correctness is hard. 
Third, voters should not have to trust the terminals they use to vote, as they may be malicious; voters should be assured their vote was recorded, without disclosing any information on how they voted to the malicious entity controlling their device.

% \subsection{Building blocks}\label{sec:blocks}
% \textbf{Verifiable linear secret sharing (VSS).} In this work, we use Pedersen's VSS~\cite{vss} to split the election data among several trustees. In a $(t,n)$-VSS, at least $t$ shares are required to reconstruct the original data, and any collection of less than $t$ shares leaks no information about the original data. Moreover, Pedersen's VSS is  additively homomorphic, i.e., one can compute the share of $a+b$ by adding the share of $a$ and the share of $b$, respectively.
% 
% \textbf{Perfectly binding commitment.} We encode the $i$-th option as $\vec{e}_i$, a unit vector where the $i$-th element is $1$ and the rest elements are $0$. The commitment of an option encoding is a vector of (lifted) ElGamal ciphertexts~\cite{ElGamal} that element-wise encrypts a unit vector. Note that this commitment scheme is also additively homomorphic, i.e. the commitment of $e_a + e_b$ can be computed by component-wise multiplying the corresponding commitments of $e_a$ and $e_b$.
% \textcolor{green}{TODO: define ``opening''}
% 
% \textbf{Zero-knowledge proofs.} We utilize the Chaum-Pedersen  zero-knowledge proof~\cite{CP} to ensure that all the posted commitments contain a valid option encoding. Namely, the prover uses Sigma OR proof to show that each ElGamal ciphertext encrypts either $0$ or $1$, and the product of the all the ciphertexts in a vector encrypts $1$.

\subsection{System overview}
\label{sec:sysoverview}
We employ an election setup component in our system, which we call the Election Authority (EA), to alleviate the voter from employing any cryptographic operations. 
The EA is tasked to initialize all remaining system components, and then gets destroyed to preserve privacy.
The \emph{Vote Collection} (VC) subsystem collects the votes from the voters during election hours, and assures them their vote was \emph{recorded-as-cast}.
Our \emph{Bulletin Board} (BB) subsystem, which is a public repository of all election-related information, is used to hold all ballots, votes, and the result, either in encrypted or plain form, allowing any party to read from it and verify the complete election process.
The VC subsystem uploads all votes to BB at election end time.
Finally, our design includes \emph{trustees}, who are persons entrusted with managing all actions needed until result tabulation and publication, including all actions supporting end-to-end verifiability.
Trustees hold the keys to uncover any information hidden in the BB, and we use threshold cryptography to make sure a malicious minority cannot uncover any secrets or corrupt the process.

% We encode the $i$-th option as $\vec{e}_i$, a unit vector where the $i$-th element is $1$ and the remaining elements are $0$. 
% The commitment of an option encoding is a vector of (lifted) ElGamal ciphertexts~\cite{ElGamal}, that element-wise encrypts a unit vector. Note that this commitment scheme is also additively homomorphic, i.e. the commitment of $e_a + e_b$ can be computed by component-wise multiplying the corresponding commitments of $e_a$ and $e_b$.
% \textcolor{green}{TODO: define ``opening'', notation for committed text}

% Our system uses the homomorphic property of the commitment scheme introduced in Section~\ref{sec:blocks} to tally the result without revealing individual choices. 
% More specifically, the $i$-th option is encoded into $(n+1)^{i-1}$, which we call \emph{option-encoding}. 
% For instance, if $m=3,n=9$, the \emph{option-encodings} of options $1,2,3$ are $1,10,100$, respectively. 
% Suppose we got $3$ votes for $\mathsf{option}_1$, $5$ votes for $\mathsf{option}_3$, the sum of the \emph{option-encodings} is $3*1+5*100=503$. 
% We commit \emph{option-encodings}, deriving \emph{option-encoding-commitments}.
% Due to the homomorphic property of the commitment scheme, we can sum the \emph{option-encoding-commitments} and obtain the tally result, $(3,0,5)$, without revealing the individual \emph{option-encodings}.

Our system starts with the EA generating initialization data for every component of our system. 
The EA encodes each election option, and \emph{commits} to it using a commitment scheme, as described below.
It encodes the $i$-th option as $\vec{e}_i$, a unit vector where the $i$-th element is $1$ and the remaining elements are $0$. 
The commitment of an option encoding is a vector of (lifted) ElGamal ciphertexts~\cite{ElGamal} over elliptic curve, that element-wise encrypts a unit vector. Note that this commitment scheme is also additively homomorphic, i.e. the commitment of $e_a + e_b$ can be computed by component-wise multiplying the corresponding commitments of $e_a$ and $e_b$.
The EA then creates a $\mathsf{vote code}$ and a $\mathsf{receipt}$ for each option.
Then, the EA prepares one ballot for each voter, with two functionally equivalent parts. 
Each part contains a list of options, along with their corresponding vote codes and receipts.
We consider ballot distribution to be outside the scope of this project, but we do assume ballots, after being produced by the EA, are distributed in a secure manner to each voter; thus only each voter knows the vote codes listed in her ballot.
%We also assume initialization data is transferred to each node of the remaining subsystems in a private manner.
We make sure vote codes are not stored in clear form anywhere besides the voter's ballot.

Our \emph{Vote Collection} (VC) subsystem collects the votes from the voters during election hours, by accepting up to one vote code from each voter. 
Our EA initializes each VC node with the vote codes and the receipts of the voters' ballots. 
However, it hides the vote codes, using a simple commitment scheme based on symmetric encryption of the plaintext along with a random salt value.
This way, each VC node can verify if a vote code is indeed part of a specific ballot, but cannot recover any vote code until the voter actually chooses to disclose it. 
Additionally, we secret-share each receipt across all VC-nodes using an $(N-f, N)$-VSS (verifiable secret-sharing) scheme with trusted dealer, making sure that a receipt can be recovered and posted back to the voter only when a strong majority of VC nodes participates successfully in our voting protocol.
With this design, our system adheres to the following contract with the voters: \emph{Any honest voter who receives a valid receipt from a Vote Collector node, is assured her vote will be published on the BB, and thus included in the election tally}.

The voter selects one part of her ballot at random, and posts her selected vote code to one of the VC nodes. 
When she receives a receipt, she compares it with the one on her ballot corresponding to the selected vote code.
If it matches, she is assured her vote was recorded and will be included in the election tally.
The other part of her ballot, the one not used for voting, will be used for auditing purposes.
This design is essential for verifiability, in the sense that the EA cannot predict which part a voter may use, and the unused part will betray a malicious EA with $1/2$ probability per audited ballot.

Our second distributed subsystem is the Bulletin Board (BB), which is a replicated service of isolated nodes.
Each BB node is initialized from the EA with vote codes and associated option encodings in committed form (again, for vote code secrecy), and each BB node provides public access to its stored information.
At election end time, VC nodes run our Vote Set Consensus protocol, which guarantees all VC nodes agree on a single set of voted vote codes.
%$\langle\mathsf{serial\textrm{-}no},\mathsf{vote\textrm{-}code}\rangle$ tuples. 
Then, VC nodes upload this set to each BB node, which in turn publishes this set once enough VC nodes provide the same set.

%Our third distributed subsystem are trustees, who are initialized by the EA with shares of the openings of the EA's commitments.
Our third distributed subsystem is a set of trustees, who are persons entrusted with managing all actions needed until result tabulation and publication, including all actions supporting end-to-end verifiability.
Secrets that may uncover information in the BB are shared across trustees, making sure malicious trustees under a certain threshold cannot disclose sensitive information.
We use Pedersen's Verifiable linear Secret Sharing (VSS)~\cite{vss} to split the election data among the trustees. 
In a $(k,n)$-VSS, at least $k$ shares are required to reconstruct the original data, and any collection of less than $k$ shares leaks no information about the original data. 
Moreover, Pedersen's VSS is  additively homomorphic, i.e. one can compute the share of $a+b$ by adding the share of $a$ and the share of $b$ respectively.
This approach allows trustees to perform homomorphic ``addition'' on the option-encodings of cast vote codes, and contribute back a share of the opening of the homomorphic ``total''. 
Once enough trustees upload their shares of the ``total'', the election tally is uncovered and published at each BB node.

Note that, to ensure voter privacy, the system cannot reveal the content inside an option encoding commitment at any point. 
However, a malicious EA might put an arbitrary value (say $9000$ votes for option $1$) inside such a commitment, causing an incorrect tally result. 
To prevent this, we utilize the Chaum-Pedersen  zero-knowledge proof~\cite{CP}, allowing the EA to show that the content inside each commitment is a valid option encoding, without revealing its actual content.
%, to ensure that all the posted commitments contain a valid option encoding. 
Namely, the prover uses Sigma OR proof to show that each ElGamal ciphertext encrypts either $0$ or $1$, and the sum of all elements in a vector is $1$.
%we use the zero knowledge proof scheme described in~\ref{sec:blocks}, allowing the EA to show that the content inside each commitment is a valid option encoding, without revealing its actual content. 
Our zero knowledge proof is organized as follows.
First, the EA posts the initial part of the proofs on the BB.
During the election, each voter's A/B part choice is viewed as a source of randomness, $0/1$, and all the voters' coins are collected and used as the challenge of our zero knowledge proof.
After that, the trustees will jointly produce the final part of the proofs and post it on the BB before the opening of the tally. 
Hence, everyone can verify those proofs on the BB. 
Due to space, we omit the zero-knowledge proof components in this paper and refer the interested reader to~\cite{CP}.% for details.
%\cite{kiayias-eurocrypt-2015} for details. 

Our design allows any voter to read information from the BB, combine it with her private ballot, and verify her ballot was included in the tally.
Additionally, any third-party auditor can read the BB and verify the complete election process.
As the number of auditors increases, the probability of election fraud going undetected diminishes exponentially.
For example, even if only $10$ people audit, with each one having $1 \over 2$ probability of detecting ballot fraud, the probability of ballot fraud going undetected is only ${1 \over 2}^{10} = 0.00097$.
Thus, even if the EA is malicious and, e.g.,  tries to point all vote codes to a specific option, this faulty setup will be detected because of the end-to-end verifiability of the complete system.

\subsection{System and threat model}
\label{subsec:threat}
We assume a fully connected network, where each node can reach any other node with which it needs to communicate. 
The network can drop, delay, duplicate, or deliver messages out of order. 
However, we assume messages are eventually delivered, provided the sender keeps retransmitting them.
For all nodes, we make no assumptions regarding processor speeds.
We assume the clocks of VC nodes are synchronized with real time; this is needed simply to prohibit voters from casting votes outside election hours. 
Besides this, we make no other timing assumptions in our system.
We assume the EA sets up the election and is destroyed upon completion of the setup, as it does not directly interact with the remaining components of the system, thus reducing the attack surface for the privacy of the voting system as a whole.
We also assume initialization data for every system component is relayed to it via untappable channels.
We assume the adversary does not have the computational power to violate any underlying cryptographic assumptions. 
To ensure liveness, we additionally assume the adversary cannot delay communication between honest nodes above a certain threshold.
We place no bound on the number of faulty nodes the adversary can coordinate, as long as the number of malicious nodes of each
subsystem is below its corresponding fault threshold. 
We consider arbitrary (Byzantine) failures, because we expect our system to be deployed across separate administrative domains. 
Let $N_v$, $N_b$, and $N_t$ be the number of VC nodes, BB nodes, and trustees respectively. 
\ifextended
The voters are denoted by $V_\ell$, $\ell=1,\ldots,n$. 
For each of the subsystems, we have the following fault tolerance thresholds:
\begin{itemize}
 \item 
The number of faulty VC nodes, $f_v$, is strictly less than $1/3$ of $N_v$, i.e., for fixed $f_v$: $$\boxed{N_v\geq3f_v+1.}$$
 \item 
The number of faulty BB nodes, $f_b$, is strictly less than $1/2$ of $N_b$, i.e., for fixed $f_b$: $$\boxed{N_b\geq2f_b+1.}$$
 \item 
For the trustees' subsystem, we apply $h_t$ out-of $N_t$ verifiable secret sharing, where $h_t$ is the number of honest trustees, thus we tolerate $f_t=N_t-h_t$ malicious trustees.  
\end{itemize}
\else
For each of the subsystems, we have the following fault tolerance thresholds:
\begin{itemize}
\item
The number of faulty VC nodes, $f_v$, is strictly less than $1/3$ of $N_v$.
\item
The number of faulty BB nodes, $f_b$, is strictly less than $1/2$ of $N_b$.
\item
For the trustees' subsystem, we apply $h_t$ out-of $N_t$ verifiable secret sharing, where $h_t$ is the number of honest trustees, thus we tolerate $f_t=N_t-h_t$ malicious trustees.  
\end{itemize}
\fi
%We assume the EA is a trusted setup component, and thus it is honest. 

%In the sections below, we go into more detail on the specifics of each subsystem.

\subsection{Election Authority}
\label{sect:EA}
EA produces the initialization data for each election entity in the setup phase. 
To enhance the system robustness, we let the EA generate all the public/private key pairs for all the system components (except voters) without relying on external PKI support.
We use zero knowledge proofs to ensure the correctness of all the initialization data produced by the EA. 

\emph{Voter ballots.} 
The EA generates one ballot $\mathsf{ballot}_\ell$ for each voter $\ell$, and assigns a unique $64$-bit $\mathsf{serial\textrm{-}no}_\ell$ to it.
As shown below, each ballot consists of two parts: Part A and Part B. 
Each part contains a list of $m$ $\langle\mathsf{vote\textrm{-}code},\mathsf{option},\mathsf{receipt}\rangle$ tuples, one tuple for each election option.
The EA generates the vote-code as a $160$-bit random number, unique within the ballot, and the receipt as $64$-bit random number.

%We call this list of tuples the \emph{lines} of the ballot.
\begin{center}
\begin{scriptsize}
	\begin{tabular}{|l l l |}
		\hline
		$\mathsf{serial\textrm{-}no}_\ell$ &  &\\
		\hline
		& Part A &\\
		$\mathsf{vote\textrm{-}code}_{\ell,1}$ & $\mathsf{option}_{\ell,1}$ & $\mathsf{receipt}_{\ell,1}$\\
		$\quad\hdots$ & $\quad\hdots$ & $\quad\hdots$\\
		$\mathsf{vote\textrm{-}code}_{\ell,m}$ & $\mathsf{option}_{\ell,m}$ & $\mathsf{receipt}_{\ell,m}$\\
		\hline
		& Part B &\\
		$\mathsf{vote\textrm{-}code}_{\ell,1}$ & $\mathsf{option}_{\ell,1}$ & $\mathsf{receipt}_{\ell,1}$\\
		$\quad\hdots$ & $\quad\hdots$ & $\quad\hdots$\\
		$\mathsf{vote\textrm{-}code}_{\ell,m}$ & $\mathsf{option}_{\ell,m}$ & $\mathsf{receipt}_{\ell,m}$\\
		\hline
	\end{tabular}
	\end{scriptsize}
\end{center}

\emph{BB initialization data.} The initialization data for all BB nodes is identical, and each BB node publishes its initialization data immediately. 
The BB's data is used to show the correspondence between the vote codes and their associated cryptographic payload.
This payload comprises the committed option encodings, and their respective zero knowledge proofs of valid encoding (first move of the prover), as described in section~\ref{sec:sysoverview}. 
However, the vote codes must be kept secret during the election, to prevent the adversary from ``stealing'' the voters' ballots and using the stolen vote codes to vote. 
To achieve this, the EA first randomly picks a $128$-bit key, $\mathsf{msk}$, and encrypts each $\mathsf{vote\textrm{-}code}$ using AES-128-CBC with random initialization vector (AES-128-CBC\$) encryption, denoted as $[\mathsf{vote\textrm{-}code}]_{\mathsf{msk}}$.
Each BB is given $H_{\mathsf{msk}}\leftarrow SHA256(\mathsf{msk} , \mathsf{salt}_\mathsf{msk})$ and $\mathsf{salt}_\mathsf{msk}$, where $\mathsf{salt}_\mathsf{msk}$ is a fresh $64$-bit random salt. Hence, each BB node can be assured the key it reconstructs from VC key-shares (see below) is indeed the key that was used to encrypt these vote-codes. 
\indent The rest of the BB initialization data is as follows: for each $\mathsf{serial\textrm{-}no}_\ell$, and for each ballot part, there is a \emph{shuffled} list of $\left\langle[\mathsf{vote\textrm{-}code}_{\ell,\pi_\ell^X(j)}]_{\mathsf{msk}},\mathsf{payload}_{\ell,\pi_\ell^X(j)} \right\rangle$ tuples, where $\pi_\ell^X\in S_m$ is a random permutation ($X$ is $A$ or $B$).
%and $\mathsf{payload}_{\ell,j}$ is the corresponding cryptographic collection. 
\ifextended
\begin{center}
\begin{scriptsize}
	\begin{tabular}{|l c|}
		\hline
		\hspace{55pt}$(H_{\mathsf{msk}}, \mathsf{salt}_\mathsf{msk})$  &\\
		\hline
		\hline
		$\mathsf{serial\textrm{-}no}_\ell$  &\\
		\hline
		& Part A \\
		$[\mathsf{vote\textrm{-}code}_{\ell,\pi_\ell^A(1)}]_{\mathsf{msk}}$ & $\mathsf{payload}_{\ell,\pi_\ell^A(1)}$  \\
		\quad\quad $\vdots$ & $\vdots$\\
		$[\mathsf{vote\textrm{-}code}_{\ell,\pi_\ell^A(m)}]_{\mathsf{msk}}$ & $\mathsf{payload}_{\ell,\pi_\ell^A(m)}$  \\
		\hline
		& Part B \\
		$[\mathsf{vote\textrm{-}code}_{\ell,\pi_\ell^B(1)}]_{\mathsf{msk}}$ & $\mathsf{payload}_{\ell,\pi_\ell^B(1)}$  \\
		\quad\quad $\vdots$ & $\vdots$\\
		$[\mathsf{vote\textrm{-}code}_{\ell,\pi_\ell^B(m)}]_{\mathsf{msk}}$ & $\mathsf{payload}_{\ell,\pi_\ell^B(m)}$  \\
		\hline
	\end{tabular}
\end{scriptsize}	
\end{center}
\fi
We shuffle the list of tuples of each part to ensure voter's privacy. 
This way, nobody can guess the voter's choice from the position of the cast vote-code in this list.

\emph{VC initialization data.} %Recall that $\underline{m}$ denotes the opening of the commitment $\Com(m)$. 
%Let $\underline{\mathsf{key}}$ be the opening of the above key commitment.
The EA uses an $(N_v-f_v,N_v)$-VSS (Verifiable Secret-Sharing) scheme to split $\mathsf{msk}$ and every $\mathsf{receipt}_{\ell,j}$, denoted as $(\|\mathsf{msk}\|_1,\ldots, \|\mathsf{msk}\|_{N_v})$ and $(\|\mathsf{receipt}_{\ell,j}\|_1,\ldots, \allowbreak\|\mathsf{receipt}_{\ell,j}\|_{N_v})$. 
For each $\mathsf{vote\textrm{-}code}_{\ell,j}$ in each ballot, the EA also computes $H_{\ell,j}\leftarrow SHA256(\mathsf{vote\textrm{-}code}_{\ell,j} , \mathsf{salt}_{\ell,j})$, where $\mathsf{salt}_{\ell,j}$ is a $64$-bit random number. 
$H_{\ell,j}$ allows each VC node to validate a $\mathsf{vote\textrm{-}code}_{\ell,j}$ individually (without network communication), while still keeping the $\mathsf{vote\textrm{-}code}_{\ell,j}$ secret. 
To preserve voter privacy, these tuples are also shuffled using $\pi_\ell^X$.
The initialization data for $VC_i$ is structured as below:
\begin{center}
\begin{scriptsize}
	\begin{tabular}{|l c|}
	    \hline
	    \multicolumn{2}{|c|}{$\|\mathsf{msk}\|_i$}\\
	    \hline
		\hline
		$\mathsf{serial\textrm{-}no}_\ell$ &  \\
		\hline
                \multicolumn{2}{|c|}{Part A} \\
		$(H_{\ell,\pi_{\ell}^A(1)},\mathsf{salt}_{\ell,\pi_{\ell}^A(1)})$  & $\|\mathsf{receipt}_{\ell,\pi_{\ell}^A(1)}\|_i$ \\
		\quad $\hdots$ & $\hdots$ \\
	$(H_{\ell,\pi_{\ell}^A(m)},\mathsf{salt}_{\ell,\pi_{\ell}^A(m)})$ & $\|\mathsf{receipt}_{\ell,\pi_{\ell}^A(m)}\|_i$\\
                \hline
                \multicolumn{2}{|c|}{Part B} \\
                $(H_{\ell,\pi_{\ell}^B(1)},\mathsf{salt}_{\ell,\pi_{\ell}^B(1)})$  & $\|\mathsf{receipt}_{\ell,\pi_{\ell}^B(1)}\|_i$ \\
                \quad $\hdots$ & $\hdots$ \\
        $(H_{\ell,\pi_{\ell}^B(m)},\mathsf{salt}_{\ell,\pi_{\ell}^B(m)})$ & $\|\mathsf{receipt}_{\ell,\pi_{\ell}^B(m)}\|_i$\\
		\hline
	\end{tabular}
	\end{scriptsize}
\end{center}

\emph{Trustee initialization data.} The EA uses $(h_t,N_t)$-VSS to split the opening of encoded option commitments $\Com(\vec{e}_i)$, denoted as $(\left[\underline{\vec{e}_i}\right]_1,\ldots, \allowbreak\left[\underline{\vec{e}_i}\right]_{N_t})$.
The initialization data for $\mathsf{Trustee}_i$ is structured as below:
\begin{center}
\begin{scriptsize}
	\begin{tabular}{|l c|}
		\hline
		$\mathsf{serial\textrm{-}no}_\ell$  &\\
		\hline
		\multicolumn{2}{|c|}{Part A}\\
		 $\Com(\vec{e}_{\pi_\ell^A(i)})$  & $\left[\underline{\vec{e}_{\pi_\ell^A(i)}}\right]_\ell$\\
		$\cdots$ & $\cdots$\\
		\hline
		\multicolumn{2}{|c|}{Part B}\\
	  $\Com(\vec{e}_{\pi_\ell^B(i)})$  & $\left[\underline{\vec{e}_{\pi_\ell^B(i)}}\right]_\ell$\\
		$\cdots$ & $\cdots$ \\
		\hline
	\end{tabular}
	\end{scriptsize}
\end{center}

Similarly, the state of zero knowledge proofs for ballot correctness is shared among the trustees using $(h_t,N_t)$-VSS. 
Due to space limitation, we omit the detailed description here and refer the reader to~\cite{CP}.


\subsection{Vote Collectors}\label{subsec:Vcnodes}
% ($N_v$)
\input{system-vc}

\subsection{Voter}\label{subsec:voter}
% ($n$)
%The voter has received her ballot from the BDS of the VCS; 
We expect the voter, who has received a ballot from EA, to know the URLs of at least $f_\mathsf{v}+1$ VC nodes.
To vote, she picks one part of the ballot at random, selects the vote code representing her chosen option, and loops, selecting a VC node at random and posting the vote code, until she receives a valid receipt. 
%follows Alg.~\ref{alg:vote}.
After the election, the voter can verify two things from the updated BB. 
First, she can verify her cast vote code is included in the tally set. 
Second, she can verify that the unused part of her ballot, as ``opened'' at the BB, matches the copy she received before the election started.
This step verifies that the vote codes are associated with the expected options as printed in the ballot.
Finally, the voter can delegate both of these checks to an \emph{auditor}, without sacrificing her privacy; this is because the cast vote code does not reveal her choice, and because the unused part of the ballot is completely unrelated to the used one.

\begin{comment}
\begin{algorithm}
\caption{Voting algorithm}
\label{alg:vote}
\begin{algorithmic}[1]
\NoThen
\scriptsize
\Procedure{Vote}{$\mathsf{ballot}$, $\mathsf{selection}$, $\mathsf{VC\textrm{-}List}$}:
  \State $\mathsf{vote\textrm{-}code}$ := $\mathsf{ballot}.\mathsf{lines}[\mathsf{selection}].\mathsf{vote\textrm{-}code}$
  \State $\mathsf{VC\textrm{-}List}$ := random-shuffle($\mathsf{VC\textrm{-}List}$)
  \Repeat
%    \For {$\mathsf{VC\textrm{-}Node}$ in $\mathsf{VC\textrm{-}List}$}
	  \State $\mathsf{VC\textrm{-}Node}$ := $\mathsf{VC\textrm{-}List}$.popFirst()
	  \State send $\mathsf{VC\textrm{-}Node}$ VOTE$( \mathsf{ballot}.\mathsf{serial\textrm{-}no}, \mathsf{vote\textrm{-}code})$
	  \State wait up to timeout for $\mathsf{receipt}$
%	\EndFor
  \Until $\mathsf{receipt}$ == $\mathsf{ballot}.\mathsf{lines}[\mathsf{selection}].\mathsf{receipt}$
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{comment}

\subsection{Bulletin Board}\label{sec:BB}
A BB node is a pubic repository of election-specific information. 
By definition, it can be read via a public and anonymous channel.
Writes, on the other hand, happen over an authenticated channel, implemented with PKI originating from the voting system.
BB nodes are independent from each other; a BB node never directly contacts another BB node.
Readers are expected to issue a read request to all BB nodes, and trust the reply that comes from the majority.
Writers are also expected to write to all BB nodes; their submissions are always verified, and explained in more detail below.
\\\indent 
After the setup phase, each BB node publishes its initialization data. 
During election hours, BB nodes remain inert.
After the voting phase, each BB node receives from each VC node, the final vote-code set and the shares of $\mathsf{msk}$.
Once it receives $f_v+1$ identical final vote code sets, it accepts and publishes the final vote code set.
Once it receives $N_v-f_v$ valid key shares (again from VC nodes), it reconstructs the $\mathsf{msk}$, decrypts all the encrypted vote codes in its initialization data, and publishes them.
%for the opening of $\Com(\mathsf{key})$, ABB reconstructs the $\mathsf{key}$ and decrypts all the vote-codes. 
%The final
%, $[\underline{\mathsf{key}}]_\ell$, the ABB node checks the attached signature and publishes them.
%
%Once receives $N_v-f_v$ valid shares for the opening of $\Com(\mathsf{key})$, ABB reconstructs the $\mathsf{key}$ and decrypts all the vote-codes. 
%The final cast vote-code list is determined by majority of the vote-code lists submitted by all the VC nodes.
%
\\\indent 
%Subsequently, a BB locates the decrypted vote codes that belong to the final cast vote code set, and marks them as ``$\mathsf{voted}$''.
At this point, the cryptographic payloads corresponding to the cast vote codes are made available to the trustees. 
Trustees, in turn, read from the BB subsystem, perform their individual calculations and then write to the BBs; these writes are verified by the trustees' keys, generated by the EA. 
Once enough trustees have posted valid data, the BB node combines them and publishes the final election result.
\\\indent
We intentionally designed our BB nodes to be as simple as possible for the reader, refraining from using a Replicated State Machine, which would require readers to run algorithm-specific software. 
The robustness of BB nodes comes from controlling all write accesses to them. 
%The initialization message comes from the EA, which is trusted and assumed to be correct.
Writes from VC nodes are verified against their honest majority threshold. 
Further writes are allowed only from trustees, verified by their keys.
\\\indent 
Finally, a reader of our BB nodes should post her read request to all nodes, and accept what the majority responds with ($f_b+1$ is enough). 
We acknowledge there might be temporary state divergence (between BB nodes), between the time a writer finishes updating one BB node, and until he updates another. 
However, given our thresholds, this should be only momentary, alleviated with simple retries.
Thus, if there is no reply backed by a clear majority, the reader should retry until there is one.
%that, the post-processing component will update each BB's election transcript by appending the final election data. (cf. Step (d) in Figure~\ref{fig:BB}.) The data usually includes the election tally as well as necessary information for verifiability.
%\vspace{-5px}
\subsection{Trustees}
After the end of election, each trustee fetches all the election data from the BB subsystem and verifies the validity of the election data. 
%The majority of view of the election transcript posted on the BB is considered as the genuine election transcript, which will be used to calculate the tally result. 
For each ballot, there are two possible valid outcomes: i) one of the A/B parts are voted, ii) none of the A/B parts are voted. 
If both A/B parts of a ballot are marked as voted, then the ballot is considered as invalid and should be discarded. 
Similar, trustees also discard those ballots where more than maximum allowed commitments in an A/B part are marked as voted.
In case (i), for each encoded option commitment in the unused part, $\mathsf{Trustee}_\ell$ submits its corresponding share of the opening of the commitment to the BB; for each encoded option commitment in the voted part, $\mathsf{Trustee}_\ell$ computes and posts the share of the final message of the corresponding zero knowledge proof, showing the validity of those commitments; meanwhile, those commitments marked as voted are collected to a tally set $\mathbf{E}_{\mr{tally}}$. 
In case (ii), for each encoded option commitment in both parts, $\mathsf{Trustee}_\ell$ submits its corresponding share of the opening of the commitment to the BB.
Finally, denote $\mathbf{D}^{(\ell)}_{\mr{tally}}$ as $\mathsf{Trustee}_\ell$'s set of shares of option encoding commitment openings,   corresponding to the commitments in $\mathbf{E}_{\mr{tally}}$.
$\mathsf{Trustee}_\ell$ computes the opening share for $E_{\mr{sum}}$ as $T_\ell = \sum_{D\in \mathbf{D}^{(\ell)}_{\mr{tally}}}$ and then submits $T_\ell$ to each BB node. 


% \subsection{Auditors}
% Auditors are participants of our system who can verify the election process. 
% The role of the auditor can be assumed by voters or any other party.
% Auditors read information from the BB and verify the correct execution of the election.
% They may also receive audit information (an unused ballot part and a cast vote code) from any voter that wishes to delegate verification. 
% After the election, the auditors fetch the election data from the BB and check the following are valid: 
% a) within each opened ballot, no two vote codes are the same; 
% b) there are no two submitted vote codes associated with any single ballot part; 
% c) within each ballot, no more than one part has been used; 
% d) the submitted vote codes are consistent with the ones received from the voters; 
% e) all the openings of the commitments are valid; 
% f) the openings of the unused ballot parts are consistent with the ones received from the voters; 
% g) all the zero-knowledge proofs that are associated with the used ballot parts are completed and valid.

\subsection{Auditors}
\label{sec:auditors}
Auditors are participants of our system who can verify the election process. 
The role of the auditor can be assumed by voters or any other party.
After election end time, auditors read information from the BB and verify the correct execution of the election, by verifying the following:
a) within each opened ballot, no two vote codes are the same; 
b) there are no two submitted vote codes associated with any single ballot part; 
c) within each ballot, no more than one part has been used; 
d) all the openings of the commitments are valid; 
e) all the zero-knowledge proofs that are associated with the used ballot parts are completed and valid;
%\\\indent
In case they received audit information (an unused ballot part and a cast vote code) from voters who wish to delegate verification, they can also verify:
f) the submitted vote codes are consistent with the ones received from the voters; 
g) the openings of the unused ballot parts are consistent with the ones received from the voters.



\begin{comment}
\subsection{Properties of Distributed DEMOS}\label{subsubsec:dDemos-properties}
Our resulting D-DEMOS voting system preserves both the end-to-end verifiability and privacy properties of centralized DEMOS.
\par\noindent\textbf{End-to-end verifiability. } Centralized DEMOS achieves end-to-end verifiability against an adversary that controls the entire election procedure (\cite[Theorem 4]{DEMOS}). Therefore, Distributed DEMOS preserves the same level of end-to-end verifiability against adversaries that may corrupt the EA, the TS, the BDS, all VC nodes, and all the trustees. 
In addition, the consistency of the view of the BB, which is the only requirement for end-to-end verifiability, is achieved by the fault tolerance threshold of the BB nodes.
%
\par\noindent\textbf{Voter privacy. } Centralized DEMOS achieves voter privacy against adversaries that observe the entire network traffic and obtain the voters' audit information (\cite[Theorem 5]{DEMOS}).  In this model, the EA, the VC and the trustees' subsystems  are merged in to a single honest authority. Adapting the proof to the system model described in Section~\ref{sec:model} is accomplished by (i) destroying the EA and DBB's TS (ii) the fault tolerance threshold of the VC and the trustees' subsystems and (iii) the fault tolerance threshold of the BB subsystem.

By integrating DEMOS with our DBB, the resulting system possesses the following extra properties:
\begin{itemize}
 \item It provides fault-tolerant long-term storage of election data, using our BB nodes.
 \item It provides fault-tolerant vote collection, during election hours, using our VC nodes.
 \item It provides immediate feedback to the voter, assuring her that her vote was recorded-as-cast, using our receipt mechanism. 
 In the original DEMOS system, the voter has to consult the BB after election hours, to verify her vote was recorded, a far more complex interaction for unsophisticated users.
\end{itemize}

Furthermore, by applying threshold cryptography and introducing \emph{trustees}, we eliminate all single points of failure, beyond the setup performed by the EA. Note that, due to the inherent end-to-end verifiability of DEMOS, a malicious setup by the EA can be detected using the \emph{Verify} algorithm. Thus, even the only remaining centralized component cannot lead to an undetected erroneous election result.
To our knowledge, Distributed DEMOS is the \textbf{first end-to-end verifiable web-based voting system without any single point of failure besides setup}.
\end{comment}


==> unsynchronous.tex <==
\section{Removing the barrier assumption}\label{sec:unsychronous}
\input{system-bc}
